LL/SC and Atomic Copy: Constant Time, Space Efficient Implementations using only pointer-width CAS

When designing concurrent algorithms, Load-Link/Store-Conditional (LL/SC) is often the ideal primitive to have because unlike Compare and Swap (CAS), LL/SC is immune to the ABA problem. However, the full semantics of LL/SC are not supported by any modern machine, so there has been a significant amount of work on simulations of LL/SC using Compare and Swap (CAS), a synchronization primitive that enjoys widespread hardware support. All of the algorithms so far that are constant time either use unbounded sequence numbers (and thus base objects of unbounded size), or require $\Omega(MP)$ space for $M$ LL/SC object (where $P$ is the number of processes). We present a constant time implementation of $M$ LL/SC objects using $\Theta(M+kP^2)$ space, where $k$ is the maximum number of overlapping LL/SC operations per process (usually a constant), and requiring only pointer-sized CAS objects. Our implementation can also be used to implement $L$-word $LL/SC$ objects in $\Theta(L)$ time (for both $LL$ and $SC$) and $\Theta((M+kP^2)L)$ space. To achieve these bounds, we begin by implementing a new primitive called Single-Writer Copy which takes a pointer to a word sized memory location and atomically copies its contents into another object. The restriction is that only one process is allowed to write/copy into the destination object at a time. We believe this primitive will be very useful in designing other concurrent algorithms as well.

==> app.tex <==

\section{Applications}
\label{sec:app}

In this section, we discuss some applications for Results \ref{result:swcopy} and \ref{result:llsc}.

\subsection{}

\subsection{Universal Construction}
\label{sec:universal}

Our technique probably applies to a bunch of other universal constructions, but we focus on one by Fatorou that combines many ideas from previous universal constructions and improves upon them.

Algorithm 1 of their paper \cite{fatourou2011highly}.

Given a sequential functional data structure $D$ with root set $R$. The variable \var{st} from the \var{State} object in \cite{fatourou2011highly} will store the roots of $D$ at that state. The \var{SimCollect} object will be implemented as a regular array of . \Hao{Write something about the operation descriptor size. You can probably use your work on multi-word registers to implement this thing. Or you can cite the LL/SC from CAS paper <- sort of like an overkill multi-word register}.  

I guess we will put $R$ in a giant LL/SC object 

\result{Universal Construction}{
\label{result:refcount}
Given a sequential functional data structure $D$ with root set $R$, there is an universal construction implementing $D$ in a linearizable manner on $P$ processes:
On $P$ processes, a concurrent stack can support insert and delete with
  \begin{enumerate}
   \item $O(P)$ worst-case time per operation,
   \item $O(Pd)$ shared space for storing descriptors in the \var{SimCollect} object
   \item $O(P^2+P|R|)$ shared space for the $O(P+|R|)$-word LL/SC variable \var{S}
   \item $O(P+|R|)$ local space per process to store a \var{State} object
   \item $O(Pd)$ local space per process to store a \var{SimCollect} object
   \item This does not count space reachable from the root sets of $D$. I.e. the space overhead compared to how much space $D$ would have used had all operations been invoked sequentially. I.e. space overhead of the universal construction.
   \item 
   \item single-word (pointer-width) read, write, and CAS.
  \end{enumerate}
}

Jayanti's algorithm supports constant time VL as long as we support constant time VL.

As long as user does not pop something off and then free it to system memory, we don't need to worry about garbage collection, but we do need to check the head pointer again after each push or pop. Wait, maybe we actually need to do a VL, first because checking head pointer requires an LL and second because there might be an ABA.

Wait hold on, the contents of a node could be read even after it has been popped. Maybe we have to solve garbage collection after all. Or we can have bit on the node indicating it has been collected.

So the universal construction should not talk about garbage collection at all. However after we apply it to the stack, we should talk about GC.
What we need is a constant time VL operation. Actually no, we just need to check that the head still points here.

We can say to do a VL after reading each node. Actually we never dereference a pointer starting from the head.

Youla describes a stack, so why can't we just use what they describe?

Lots of the bounds in the universal construction can be improved upon. For example descriptors can be implemented with indirection and GC. We might be able to get away with O(P) space overhead rather than O(P^2). <- actually that one not so much.
Maybe we should just implement our stack directly with the boudns we want.

\result{O(P)-time Stack}{
\label{result:refcount}
On $P$ processes, a concurrent stack can support insert and delete with
  \begin{enumerate}
   \item $O(P)$ worst-case time per operation,
   \item single-word (pointer-width) read, write, and CAS.
  \end{enumerate}
}

We need to implement a stack where push takes a pointer to a node as argument and pop returns a pointer to the node that was removed. 

\result{Fixed-sized Allocate/Free}{
\label{result:refcount}
On $P$ processes, we can support allocation and free for fixed sized blocks of $k$ words, and assuming
a maximum $m$ live blocks, with
  \begin{enumerate}
   \item references are just pointers to the block (i.e., memory addresses),
   \item $O(1)$ worst-case time for each operation,
   \item $mk + O(P^2k)$ space,
   \item single-word (pointer-width) read, write, and CAS.
  \end{enumerate}
}


==> todo.tex <==

\section{Potentially contraversal decisions}

\begin{itemize}
  \item decided not to talk about dynamically adding announcement array slots.
  \item decided not to cite memory management or reference counting paper to avoid circular reference, which would ruin double blindness
  \item Decided to stick with submitting to SPAA
\end{itemize}

\section{LL/SC paper}

\begin{itemize}
  \item add discussion of applications:
  \begin{itemize}
    \item Cite applications of swcopy: 
    \begin{itemize}
      \item other paper for constant time reference counting, memory management, and resource ownership
      \item Swcopy can be used in other algorithms to simplify the proofs. Many algorithms reinvent it and have to prove it as part of a bigger algorithm.
    \end{itemize}
    \item Cite prior work that uses LL/SC
    \begin{itemize}
      \item Faith's counter
      \item Woefel's bounded counter work?
      \item In most of this work, the number of outstanding LLs per process is bounded.
    \end{itemize}
    \item Cite work that uses CAS and unbounded sequence numbers:
    \begin{itemize}
      \item Universal constructions - Youla's previous paper. This modified version of the universal construct is used in another paper on Constant Time Memory Allocation.
      \item Garbage collection papers
      \item Work stealing scheduler
    \end{itemize}
  \end{itemize}
  \item Maybe add the refernce counting + gc algorithm for large $k$ here. It won't have as good space complexity. 
\end{itemize}

\section{Memory Allocation Paper}

\begin{itemize}
  \item Generalize theorem for universal construction and apply it to functional data structures
  \item Present a functional stack.
  \item Talk about applications (listed in another document)
  \item Combined with reference counting, this can be used to implement LL/SC where the number of LLs per process is unbounded.
\end{itemize}

\section{Memory Mangement for wait-free stack}

Options:

\begin{itemize}
  \item Disallow user from freeing the memory we return back to main memory. This feature could be nice because it allows the user to grow and shrink the memory pool. In this case we just need to call VL push and pops.
  \item Allow user to free memory back to main memory and use hazard pointers. There are two options from here. You can chop off the head of a block and store it separately if you see it is reserved. I prefer this approach because it sounds more efficient and it strengthens are arguement that we can't use previous stacks because they don't handle memory reclamantion. Or you can use another universal construction like thing to implement a global retired list. Actually no that becomes kind of circular because you'll need to implement the retired list as another stack, or maybe just an array of 2P elements.
  \item I wonder how Fatorou and Guy handle this problem. Should be ready to explain difference between this and previous wait-free stacks.
\end{itemize}

\section{Universal Construction}

Let's shift focus away from improving universal constructions. Other than removing the need for unbounded sequence numbers and possibly combining them with function data structures, we do not do much. There is still quite a lot to be done though in terms of memory management and supporting descriptors through indirection, but I think that's a topic for a later paper.

\section{Meeting with Guy}

\begin{itemize}
  \item For memory allocation, block size needs to at least be able to store two pointers. Briefly describe how you would get around this requirement
  \item Decided on a version of the algorithm.
  \item Guy supports having a single snapshot object
  \item Abstraction function can be to a different abstract state A' that is a subset of the original abstract state
  \item Abstraction function can be lazily computed given a root set
  \item There are only two types of objects, immutable tuples and handles to CAS objects.
  \item Interface that Guy suggested for snapshot objects. 
\end{itemize}
